One-Stage Cascade Refinement Networks for Infrared Small Target Detection

Single-frame InfraRed Small Target (SIRST) detection has been a challenging task due to a lack of inherent characteristics, imprecise bounding box regression, a scarcity of real-world datasets, and sensitive localization evaluation. In this paper, we propose a comprehensive solution to these challenges. First, we find that the existing anchor-free label assignment method is prone to mislabeling small targets as background, leading to their omission by detectors. To overcome this issue, we propose an all-scale pseudo-box-based label assignment scheme that relaxes the constraints on scale and decouples the spatial assignment from the size of the ground-truth target. Second, motivated by the structured prior of feature pyramids, we introduce the one-stage cascade refinement network (OSCAR), which uses the high-level head as soft proposals for the low-level refinement head. This allows OSCAR to process the same target in a cascade coarse-to-fine manner. Finally, we present a new research benchmark for infrared small target detection, consisting of the SIRST-V2 dataset of real-world, high-resolution single-frame targets, the normalized contrast evaluation metric, and the DeepInfrared toolkit for detection. We conduct extensive ablation studies to evaluate the components of OSCAR and compare its performance to state-of-the-art model-driven and data-driven methods on the SIRST-V2 benchmark. Our results demonstrate that a top-down cascade refinement framework can improve the accuracy of infrared small target detection without sacrificing efficiency. The DeepInfrared toolkit, dataset, and trained models are available at https://github.com/YimianDai/open-deepinfrared to advance further research in this field.

==> contents/biography.tex <==
% !TEX root = ../main.tex

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./figs/photo/Yimian}}]{Yimian Dai} received his Ph.D. in signal and information processing from Nanjing University of Aeronautics and Astronautics in 2020. During his doctoral studies, he was a visiting Ph.D. student at the University of Copenhagen from March 2018 to September 2018, and at the University of Arizona from October 2018 to October 2020. He is currently a post-doctoral researcher at Nanjing University of Science and Technology, where his research focuses on remote sensing, computer vision, and deep learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/photo/Yaohong}}]{Yaohong Chen} received his B.E. from Fourth Military Medical University in 2010 and his M.E. from Xi'an Jiaotong University in 2013. He is currently an engineer at the Xi'an Institute of Optics and Precision Mechanics, Chinese Academy of Sciences, and a Ph.D. candidate at the University of Chinese Academy of Sciences since 2018. During his doctoral studies, he was a visiting Ph.D. student at the Johns Hopkins University from September 2019 to August 2020. His research interests include the development of infrared imaging systems, infrared image processing, and infrared target detection.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/photo/Xiang}}]{Xiang Li} received the PhD degree from the Department of Computer Science and Technology, Nanjing University of Science and Technology (NJUST) in 2020. 
  
  In 2016, he spent eight months as a research intern in Microsoft Research Asia.
  Dr. Li started his postdoctoral career in NJUST as a candidate for the 2020 Postdoctoral Innovative Talent Program. 
  He is also a long-term visiting scholar at Momenta, working on monocular perception algorithm.

  His recent works mainly focus on monocular perception, object detection/recognition, unsupervised learning, big data, and neural architecture design.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.35in,clip,keepaspectratio]{./figs/photo/Feifei}}]{Feifei Zhang} received the Ph.D. degree from the State Key Laboratory of Information Engineering in Surveying, Mapping and Remote Sensing, Wuhan University, Wuhan, China, in 2015. 

  She is currently a lecturer with the School of Computer Science in Guang Dong University of Education, GuangZhou, China. Her current research interests include computer vision, remote sensing, and machine learning.
  
\end{IEEEbiography}

\begin{IEEEbiography}[{
  \includegraphics[width=1.45in,height=1.3in,clip,keepaspectratio]{./figs/photo/Jian}}]{Jian Yang} received the Ph.D. degree in pattern recognition and intelligence systems from the Nanjing University of Science and Technology (NJUST), Nanjing, China, in 2002.

  In 2003, he was a Post-Doctoral Researcher with the University of Zaragoza, Zaragoza, Spain. From 2004 to 2006, he was a Post-Doctoral Fellow with Biometrics Centre, The Hong Kong Polytechnic University, Hong Kong. From 2006 to 2007, he was a Post-Doctoral Fellow with the Department of Computer Science, New Jersey Institute of Technology, Newark, NJ, USA.

  He is currently a Chang-Jiang Professor with the School of Computer Science and Engineering, NJUST.
  He is the author of more than 300 scientific articles in pattern recognition and computer vision.
  His journal articles have been cited more than 9600 times in the ISI Web of Science and 24400 times in the Web of Scholar Google. His research interests include pattern recognition, computer vision, and machine learning.

  Dr. Yang is a fellow of International Association for Pattern Recognition (IAPR).
  He has been an Associate Editor of \textit{Pattern Recognition Letters}, the \textsc{IEEE Transactions on Neural Networks and Learning Systems}, and \textit{Neurocomputing}.
\end{IEEEbiography}

